EvoGrad: A Dynamic Take on the Winograd Schema Challenge with Human Adversaries

While Large Language Models (LLMs) excel at the Winograd Schema Challenge (WSC), a coreference resolution task testing common-sense reasoning through pronoun disambiguation, they struggle with instances that feature minor alterations or rewording. To address this, we introduce EvoGrad, an open-source platform that harnesses a human-in-the-loop approach to create a dynamic dataset tailored to such altered WSC instances. Leveraging ChatGPT's capabilities, we expand our task instances from 182 to 3,691, setting a new benchmark for diverse common-sense reasoning datasets. Additionally, we introduce the error depth metric, assessing model stability in dynamic tasks. Our results emphasize the challenge posed by EvoGrad: Even the best performing LLM, GPT-3.5, achieves an accuracy of 65.0% with an average error depth of 7.2, a stark contrast to human performance of 92. 8% accuracy without perturbation errors. This highlights ongoing model limitations and the value of dynamic datasets in uncovering them.

==> table_archives.tex <==

% \begin{table*}[ht]
% \small 
% \begin{center}
% \begin{tabular}{L{4.5cm}L{4.5cm}L{1.5cm}L{1.5cm}L{1cm}}
% \toprule
% \multicolumn{5}{l}{\textbf{Sentence $s_0$}: I poured water from the bottle into the cup until the _ was full.} \\ \bottomrule 
% \toprule

% Perturbations & Sentence & Prediction & True Label & Depth  \\

% \midrule

% \centering$s_0$ & I poured water from the bottle into the cup until the _ was full. & cup & cup & 0 \ \textcolor{green}{\ding{51}} \\

% \midrule
% \hfil$s_{1(10)} = per_{10}(s_0,\text{because})$ & I poured water from the bottle into the cup \underline{because} the _ was full. & bottle & bottle & 1 \ \textcolor{green}{\ding{51}}\\
%     \midrule
%     \hfil$s_{1(14)} = per_{14}(s_0,\text{empty})$ & I poured water from the bottle into the cup until the _ was \underline{empty}. & bottle & bottle & 1 \ \textcolor{green}{\ding{51}} \\
%     \midrule
%     \centering \hfil$s_{2(10,14)} = per_{14}(s_{1(10)},\text{empty}) = per_{10}(s_{1(14)},\text{because})$ & I poured water from the bottle into the cup \underline{because} the _ was \underline{empty}. & bottle & cup &  \textbf{2} \ \textcolor{red}{\ding{55}} (\textit{ED}=2) \\
%     \bottomrule

% \end{tabular}
% \caption{Instance construction via perturbations from Eq.\ref{perturbation_equation} on a WSC273 example, with predictions corresponding to RoBERTa fine-tuned on Winogrande-XL. Since an incorrect prediction occurs at $s_2$, with a sentence corresponding to two modified tokens from the original, it corresponds to an error depth (\textit{ED}) of 2.}
% \label{tab:running_example}
% \end{center}
% \end{table*}

% \begin{table}[hbt]
%     \centering
%     \small
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{ c c c c c }%{C{2cm}C{0.7cm}C{1cm}C{1cm}C{1cm}}
%         \toprule
%         & \textbf{Accuracy} & \multicolumn{3}{l}{\textbf{MED Statistics}} \\
%         \midrule
%         \textbf{Version} & \textbf{\corpusname{}} & %\textbf{Batch} &
%         \textbf{Average} & \textbf{High} & \textbf{Low}\\
%         \midrule
%         BERT Out-of-box & 50.6 & 0.357 & 1 & 0 \\
%         \cmidrule{2-5}
%          BERT + Winogrande & 79.7 & 3.00 & 7 & 1 \\
%          % & 96.7 & 4.5 & 7 & 1 \\
%          % & \multirow{2}{*}{Winogrande + first batch} & \multirow{2}{*}{62.8} & 85.5 & First & 3.56 & 7 & 1 \\
%          % \cmidrule{4-8}
%          % & & & 69.2 & Second & 2.00 & 6 & 1 \\
%         \midrule
%         RoBERTa Out-of-box & 50.6 & 0.357 & 1 & 0 \\
%         \cmidrule{2-5}
%          RoBERTa + Winogrande & 85.7 & 3.43 & 7 & 1 \\
%          % & 95.1 & 4.29 & 7 & 1 \\
%          % & \multirow{2}{*}{Winogrande + first batch} & \multirow{2}{*}{76.1} & 91.5 & 3.78 & 7 & 1 \\
%          % \cmidrule{4-8}
%          % & & & 80.0 & Second & 2.8 & 6 & 1 \\
%         \bottomrule
%     \end{tabular}}
%     \caption{Accuracy and MED on \corusname{} for different fine-tuning stages of BERT and RoBERTa.}
%     \label{tab:results_evograd}
% \end{table}


% \begin{table*}[ht]
% \small 
% \begin{center}
% \begin{tabular}{L{4.8cm}L{4cm}L{0.8cm}L{1.3cm}L{1.3cm}L{1.4cm}}
% \toprule
% %\multicolumn{5}{l}{\textbf{Sentence $s_0$}: I poured water from the bottle into the cup until the _ was full.} \\ \bottomrule 
% %\toprule

% Original Sentence & Perturbed Sentence & Depth & BERT & RoBERTa & True Label  \\

% \midrule

% The home that my parents had when I was in school was a lot nicer than my house now because it was sophisticated. & The home that my parents had when I was \underline{a} \underline{kid} was \underline{way} \underline{worse} than my house now because it \underline{is} \underline{revolutionary}. & 6 & house \ \textcolor{green}{\ding{51}} & house \ \textcolor{green}{\ding{51}} & house \\
%     \midrule

% Kevin yelled at Jim because he was so upset. & Kevin yelled at Jim \underline{although} he was so \underline{nice}. & 2 & Kevin \ \textcolor{green}{\ding{51}} & Jim \ \textcolor{red}{\ding{55}} & Kevin \\

% \midrule
% I poured water from the bottle into the cup until it was full. & I poured water from the bottle into the cup \underline{because} it was full. & 1 & cup \ \textcolor{red}{\ding{55}} & bottle \ \textcolor{green}{\ding{51}} & bottle \\
%     \midrule
    
%     The lawyer asked the witness a question, but he was reluctant to answer it. & The lawyer asked the witness a question, but he was reluctant to \underline{repeat} it. & 1 & witness \ \textcolor{red}{\ding{55}} & witness \ \textcolor{red}{\ding{55}} & lawyer \\
%     \bottomrule

% \end{tabular}
% \caption{Comparison of label predictions of BERT and RoBERTa (one example per case) fine-tuned on Winogrande.}
% \label{tab:model_comparison}
% \end{center}
% \end{table*}

% \begin{table*}[ht]%[hbt]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{ |l|l|l|l|l|l|}
%         \hline
%         \textbf{Model} & \textbf{Trained on} & \textbf{Wino-valid} & \textbf{\corpusname{}-M-val} & \textbf{\corpusname{}-L-val} & \textbf{\corpusname{}-test}\\
%         \hline
%         BERT & Wino & 62.75 & 71.3 & 73.8 & 94.1 \\
%         & Wino + \corpusname{}-M & 63.06 & 74.3 & - & 93.6 \\
%         & Wino + \corpusname{}-L & 62.98 & - & 70.9 & 93.6 \\
%         \hline
%         RoBERTa & Wino & 76.09 & 96.5 & 94.7 & 97.5 \\
%         & Wino + \corpusname{}-M & 76.09 & 96.5 & - & 97.5 \\
%          & Wino + \corpusname{}-L & 76.64 & - & 95.6 & 96.5 \\
%         \hline
%         ALBERT & Wino & 64.64 & 83.2 & 81.0& 93.1 \\
%         & Wino + \corpusname{}-M & 64.48 & 83.2 & - & 93.1 \\
%         & Wino + \corpusname{}-L & 64.64 & - &79.5 & 94.1 \\
%         \hline
        
%     \end{tabular}}
%     \caption{
%     Accuracy results of models on Winogrande-valid and \corpusname{} sets after training on Winogrande-XL and \corpusname{}-train.\tablefootnote{Refer to the first part of the Discussion section for reasons on RoBERTa's high accuracy.}}
%     \label{tab:results_accuracy}
% \end{table*}

% \begin{table*}[ht]%[hbt]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{ |l|l|l|l|l|}
%         \hline
%         \textbf{Model} & \textbf{Trained on} & \textbf{\corpusname{}-M-val} & \textbf{\corpusname{}-L-val} & \textbf{\corpusname{}-test} \\
%         \hline
%         BERT & Wino & 7.302 & 7.258 & 3.583 \\
%         & Wino + \corpusname{}-M & 7.308 & -& 3.538 \\
%         & Wino + \corpusname{}-L & - & 7.232 & 3.538 \\
%         \hline
%         RoBERTa & Wino & 6.286 & 6.393 & 3.800 \\
%         & Wino + \corpusname{}-M & 6.286 & - & 3.800 \\
%          & Wino + \corpusname{}-L & - & 6.652 & 4.286 \\
%         \hline
%         ALBERT & Wino & 7.971 & 7.670 & 3.643 \\
%         & Wino + \corpusname{}-M & 8.000 & - & 3.929 \\
%         & Wino + \corpusname{}-L & - & 7.694 & 3.75 \\
%         \hline
        
%     \end{tabular}}
%     \caption{Average error depths on \corpusname{} sets after training on Winogrande-XL and \corpusname{}-train.}
%     \label{tab:results_ed}
% \end{table*}

% \begin{table*}[ht]%[hbt]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{ |l|l|l|l|l|}
%         \hline
%         \textbf{Model} & \textbf{Trained on} & \textbf{\corpusname{}-M-val} & \textbf{\corpusname{}-L-val} & \textbf{\corpusname{}-test} \\
%         \hline
%         BERT & Wino & --NN (92), --JJ (62), +NN( 61) & --NN (365), +NN (294), --JJ (228) & ~NN (9), +NN (9), --NN(9) \\
%         & Wino + \corpusname{}-M & --NN (108), +NN (90), --JJ (78) & -& +NN (11), --NN (10), ~NN (9) \\
%         & Wino + \corpusname{}-L & - & --NN (373), +NN (303), --JJ (233) & +NN (11), --NN (10), ~NN (9) \\
%         \hline
%         RoBERTa & Wino & --NN (17), +NN (12), --JJ (11) & --NN (76), +NN (54), --JJ (41) & +NN (5), ~NN(4), --NN (3) \\
%         & Wino + \corpusname{}-M & --NN (17), +NN (12), --JJ (11) & - &  +NN (5), ~NN(4), --NN (3) \\
%          & Wino + \corpusname{}-L & - & --NN (61), +NN (43), --IN (32) & +NN (8), ~NN (6), --NN (5) \\
%         \hline
%         ALBERT & Wino & --NN (92), --JJ (62), +NN (61) & --NN (272), +NN (208), --JJ (169) & +NN (21), --NN (20), +JJ (13)\\
%         & Wino + \corpusname{}-M & --NN (92), --JJ (62), +NN (61) & - & +NN (22), --NN (22), +JJ (11) \\
%         & Wino + \corpusname{}-L & - & --NN (294), +NN (220), --JJ (183) & +NN (17), --NN (17), +JJ (10) \\
%         \hline
        
%     \end{tabular}}
%     \caption{Top 3 perturbations and their count on incorrect predictions on \corpusname{} sets after training on Winogrande-XL and \corpusname{}-train.}
%     \label{tab:results_perturbations}
% \end{table*}
